Holant* Dichotomy on Domain Size 3: A Geometric Perspective

Holant problems are a general framework to study the computational complexity of counting problems. It is a more expressive framework than counting constraint satisfaction problems (CSP) which are in turn more expressive than counting graph homomorphisms (GH). In this paper, we prove the first complexity dichotomy of $\mathrm{Holant}_3(\mathcal{F})$ where $\mathcal{F}$ is an arbitrary set of symmetric, real valued constraint functions on domain size $3$. We give an explicit tractability criterion and prove that, if $\mathcal{F}$ satisfies this criterion then $\mathrm{Holant}_3(\mathcal{F})$ is polynomial time computable, and otherwise it is \#P-hard, with no intermediate cases. We show that the geometry of the tensor decomposition of the constraint functions plays a central role in the formulation as well as the structural internal logic of the dichotomy.

==> sections/conclusion.tex <==
%! Tex root : ../main.tex
\section{Conclusion} 



==> sections/introfull.tex <==
%! Tex root : ../main.tex
\section{Introduction}
Holant problems were introduced in \cite{cai_computational_2011} as a broad framework to study the computational complexity of counting problems.
Counting CSP  is a special case of Holant problems~\cite{Creignou1996ComplexityOG, bulatov-dalmau-csp, 10.1145/2528400, doi:10.1137/070690201, 10.1145/1536414.1536511, DBLP:journals/siamcomp/DyerR13, 5959820, Cai2011ComplexityOC}.
In turn, counting CSP includes counting graph homomorphisms (GH),
introduced by Lov\'asz~\cite{Lovsz1967OperationsWS, Hell2004GraphsAH},
which is a special case with a single binary constraint function.
Typical Holant problems include counting all matchings, counting
perfect matchings \#PM (including all weighted versions), counting cycle
covers, counting edge colorings, and many other natural problems.
It is strictly more expressible than GH; for example, it is known that
\#PM cannot be expressed in the framework of GH~\cite{Freedman2004ReflectionPR,DBLP:journals/cpc/CaiG22}.
%%%%% added
%%%Jin-Yi Cai, Artem Govorov:
%%%Perfect matchings, rank of connection tensors and graph homomorphisms. 
%%%Comb. Probab. Comput. 31(2): 268-303 (2022)

The complexity classification program of counting problems is to classify as broad a class of  problems as possible
according to their inherent computational complexity within these
frameworks.
Let $\mathcal{F}$ be a set of (real or complex valued) constraint functions defined on some domain set $D$.
It defines a Holant problem $\hol(\mathcal{F})$ as follows.
An input consists of a graph $G = (V, E)$, where each $v \in V$ has an associated $\mathbf{F} \in \mathcal{F}$, with incident edges to $v$ labeled as input variables of $\mathbf{F}$.
The output is the sum of products of evaluations of the constraint functions over all assignments over $D$ for the variables.
The goal of the complexity classification of Holant problems is to classify the complexity of $\hol(\mathcal{F})$.
A complexity dichotomy theorem for counting problems classifies every problem
in a broad class of problems $\mathcal{F}$ 
%of certain restricted classes 
to be either polynomial time solvable or \sph.

There has been tremendous progress in the classification of 
counting GH and counting CSP~\cite{Creignou1996ComplexityOG, doi:10.1137/070690201, 10.1145/1536414.1536511,
10.1145/2528400, DBLP:journals/siamcomp/DyerR13, 5959820, Cai2011ComplexityOC, 
dyer-graph-hom,
bulatov_complexity_2005, goldberg-partition,  hutchison_graph_2010}.
%%% Need to cite GH dichotomies.
Much progress was also made in the classification of 
Holant problems, particularly on the Boolean domain ($|D|=2$), 
%%% for 15 page version omit this
i.e., when variables take 0-1 values (but constraint functions take
arbitrary values, such as partition functions from
statistical physics). This includes the
dichotomy for all complex-valued symmetric constraint functions~\cite{complex-symmetric-holant-dichotomy}
%%%%% added
%%% cite Cai Guo Williams
and for all real-valued not necessarily symmetric constraint functions~\cite{real-holant-dichotomy}.
%%%%%% added
%%% cite Shao-Cai
On the other hand, obtaining higher domain Holant dichotomy has been far more challenging.
Toward proving 
these dichotomies one often first considers restricted classes of
Holant problems assuming some particular set of constraint functions
are present. Two particularly useful sets are the equality functions
 ${\cal EQ}$ of all arities,
and all unary functions ${\cal U}$ (i.e., functions of arity one).

%Denote by ${\cal EQ}$ the set of equality functions of all arities.
%Then t
%%%%%%%%%%%% for 15 p, simplify below
The class of all counting CSP problems \#CSP($\mathcal{F})$ is exactly 
$\hol(\mathcal{F}
\cup {\cal EQ})$; i.e., counting CSP problems are the special case of Holant problems
with  ${\cal EQ}$ assumed to be included among the constraint functions. 
In this paper we study
$\holts(\mathcal{F}) = \hol_3(\mathcal{F} \cup \mathcal{U})$,
for an arbitrary set $\mathcal{F}$ of symmetric real-valued  constraint functions
on domain size 3.
(The notation $\hol^*$ denotes that all unary  constraint functions are present.)


Previously there were only two significant Holant dichotomies on higher domains.
One is for
a single ternary constraint function that has a strong symmetry property
called domain permutation invariance~\cite{cai_complexity_2016}. That work also 
solves a decades-old open problem of
the complexity of counting edge colorings. The other is a
dichotomy for $\holts(f)$ where $f$ is a single symmetric complex-valued
ternary constraint function on 
domain size 3~\cite{cai_dichotomy_2013}. Extending this
dichotomy to an arbitrary constraint function, or more ambitiously,
to a set of constraint functions has been a goal for more than 
10 years without much progress.

In this paper, we extend the $\holts$ dichotomy on domain size $3$ of \cite{cai_dichotomy_2013} to an arbitrary
set of real-valued symmetric constraint functions.
In~\cite{liu_restricted_nodate}
%(Theorem 2 of \cite{liu_restricted_nodate}), 
an interesting observation was made that an exceptional form of 
complex-valued tractable constraint functions %(form 3 in Theorem 3.1 of \cite{cai_dichotomy_2013}) 
does not occur when the function is 
%assumed to be 
real-valued.
By restricting ourselves to a set  $\mathcal{F}$ of 
%symmetric, 
real-valued constraint functions, we can bypass a lot  of difficulty
associated with this exceptional form.
Another major source of intricacy is related to the interaction of binary constraint functions
with other constraint functions in  $\mathcal{F}$.
We introduce a new geometric perspective that provides 
%insight and 
a unifying
principle in the formulation as well as
a structural internal logic of what leads to tractability and what  leads  
to \#\P-hardness. After discovering some new tractable classes of functions
aided by the geometric perspective, we 
are able to prove a $\holts(\mathcal{F})$ dichotomy.
This dichotomy is dictated by the geometry of the tensor decomposition of constraint functions.
%Although we do not get an explicit combinatorial construction as the Fibonacci gates in the Boolean domain symmetric $\holts$ dichotomy \cite{cai_complexity_2017},
%we see that a geometric perspective can help us understand the dichotomy.

% ADD the set $\mathcal{G}$: can be viewed as the orbit of the monoid action of the binary signatures on ternary signatures, or as a gadget closure.
Suppose $\mathbf{G}$ is a binary constraint function and $\mathbf{F}$ is a tenary constraint function, with $\mathbf{F} = \mathbf{u}\teh + \mathbf{v}\teh$ its tensor decomposition.
One of the simplest constructions possible with $\mathbf{G}$ and $\mathbf{F}$ is to connect $\mathbf{G}$ at the three edges of $\mathbf{F}$;
the resulting constraint function is $\mathbf{G} \teh \mathbf{F}$ which has tensor decomposition $(\mathbf{G} \mathbf{u})\teh + (\mathbf{G} \mathbf{v})\teh$.
% This suggests that we may analyze how $\mathbf{G}$ acts on the vectors $\mathbf{u}$ and $\mathbf{v}$.
We see that this gadget construction plays nicely with the tensor decomposition.
Generalizing this idea, suppose $\mathcal{B}$ is a set of binary constraint functions and $\mathcal{T}$ is a set of ternary constraint functions.
Let $\langle \mathcal{B} \rangle$ be the monoid generated by $\mathcal{B}$.
We may consider the orbit  $\mathcal{O}$ of $\mathcal{T}$ under the monoid action of $\langle \mathcal{B} \rangle$,
%denoted $\mathcal{O}$,
such that $\mathbf{G} \in \langle \mathcal{B} \rangle$ acts on $\mathbf{F} \in \mathcal{T}$ by $\mathbf{G} : \mathbf{F} \mapsto \mathbf{G}\teh \mathbf{F}$.
Although the constraint functions in $\mathcal{O}$ are the results of a very simple gadget construction, we show that $\mathcal{O}$ contains sufficient information about the interaction of  binary constraint functions and  other constraint functions, and the simplicity allows us to analyze it by considering the geometry of the vectors of the tensor decomposition of the constraint functions in $\mathcal{O}$.

% ADD the different approach for higher arity \\
Compared to the Boolean domain, 
the dichotomy theorem (\cref{thm:dichotomy-set-of-domain-3})
we wish to prove has a more abstract
%non-explicit 
form. This is informed by the
geometric perspective, but it also causes some difficulty in its proof,
%especially when trying to extend from a single ternary constraint function
when we try to extend
to a set of constraint functions of arbitrary arities.
%the non-explicit form of the existing dichotomy theorem of a single ternary constraint function is extending the dichotomy for constraint functions of higher arity.working with binary functions and the non-explicit form of the existing dichotomy theorem of a single ternary constraint function is extending the dichotomy for constraint functions of higher arity.
We introduce a new  technique   to overcome this difficulty.
 First (and this is quite a surprise), it turns out that a dichotomy of two constraint functions of arity $3$ is easier to state and prove than the dichotomy of one binary and one ternary constraint functions. Also they can be proven independently of each other.
% This is a surprise, and
This is a departure from all previous proofs of dichotomy theorems in this area.
Second, using the unary constraint functions available in $\hols$, any symmetric constraint function $\mathbf{F}$ of arity $4$  defines a linear transformation from $\mathbb{R}^3$ to the space of symmetric constraint functions of arity $3$, which corresponds to the ternary constraint functions constructible by connecting a unary function to $\mathbf{F}$.
In particular, the image of this map, $\mathscr{F}$, is a linear subspace. 
Considering the space $\mathscr{F}$ instead of specific subsignatures allows us to bypass the difficulty from the non-explicit form of the  dichotomy
statement, which is  in terms of tensor decompositions up to 
an orthogonal transformation.
%%% JSI: this is already said above
% To go around the intricacy of binary constraint functions, we instead show a dichotomy of two ternary constraint functions, which is easier to state and prove. 
We show that a dichotomy of two ternary constraint functions and the fact that $\mathscr{F}$ is closed under linear combinations imply that $\mathscr{F}$ must be of a very special form for $\holts(\mathscr{F})$ to be tractable, which in turn implies that $\mathbf{F}$ must possess a certain regularity.

While the tractability criterion in
 \cref{thm:dichotomy-set-of-domain-3} is stated in a conceptual and succinct way,
 the tractable cases are actually quite rich and varied. We present here a specific example of a new tractable case.
Denote the domain by  $D = \{\db, \dg, \dr\}$.
 %to denote the domain elements.
We use the notation in \cref{fig:ternary-signature-notation} to denote a symmetric ternary signature on domain $D$.
\begin{figure}
  \centering
\tersig{0.7}{f_{\db\db\db} f_{\db\db\dg} f_{\db\db\dr} f_{\db\dg\dg} f_{\db\dg\dr} f_{\db\dr\dr} f_{\dg\dg\dg} f_{\dg\dg\dr} f_{\dg\dr\dr} f_{\dr\dr\dr}}
\caption{Notation for expressing a symmetric ternary domain $3$ signature}
\label{fig:ternary-signature-notation}
\end{figure}
%where $f_{i j k}$ is the value of $\mathbf{F}(i,j,k)$.
Consider the four constraint functions $\mathbf{F}, \mathbf{G}, \mathbf{H}$ and $ \mathbf{B}$ in \cref{fig:f-g-h-tractable}.
%The notation is defined in \cref{subsec:notations}.
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.35\textwidth}
    \centering
  \begin{tikzpicture}[scale=0.7]
  \node at (0, 0) {$1$};
  \node at (-1, -1) {$0$};
  \node at (1, -1) {$0$};
  \node at(-2, -2) {$1$};
  \node at (0, -2) {$0$};
  \node at (2, -2) {$0$};
  \node at (-3, -3) {$0$};
  \node at (-1, -3) {$0$};
  \node at (1, -3) {$0$};
  \node at (3, -3) {$0$};
\end{tikzpicture}
\caption{$\mathbf{F}$}
\end{subfigure}
\hspace{0.1\textwidth}
\begin{subfigure}[b]{0.35\textwidth}
  \centering
  \begin{tikzpicture}[scale=0.7]
  \node at (0, 0) {$1$};
  \node at (-1, -1) {$1$};
  \node at (1, -1) {$0$};
  \node at(-2, -2) {$1$};
  \node at (0, -2) {$0$};
  \node at (2, -2) {$-2$};
  \node at (-3, -3) {$1$};
  \node at (-1, -3) {$0$};
  \node at (1, -3) {$-2$};
  \node at (3, -3) {$0$};
\end{tikzpicture}
\caption{$\mathbf{G}$}
\end{subfigure}
\\ \hfill \\
\begin{subfigure}[b]{0.35\textwidth}
  \centering
  \begin{tikzpicture}[scale=0.7]
  \node at (0, 0) {$1$};
  \node at (-1, -1) {$-1$};
  \node at (1, -1) {$0$};
  \node at(-2, -2) {$1$};
  \node at (0, -2) {$0$};
  \node at (2, -2) {$-2$};
  \node at (-3, -3) {$-1$};
  \node at (-1, -3) {$0$};
  \node at (1, -3) {$-2$};
  \node at (3, -3) {$0$};
\end{tikzpicture}
\caption{$\mathbf{H}$}
\end{subfigure} 
\hspace{0.1\textwidth}
\begin{subfigure}[b]{0.35\textwidth}
  \centering
  \begin{tikzpicture}[scale=0.7]
  \node at (0, 0) {$1$};
  \node at (-1, -1) {$0$};
  \node at (1, -1) {$0$};
  \node at(-2, -2) {$-1$};
  \node at (0, -2) {$0$};
  \node at (2, -2) {$1$};
\end{tikzpicture}
\caption{$\mathbf{B}$}
\end{subfigure}
  \caption{Four constraint functions $\mathbf{F}$, $\mathbf{G}$, $\mathbf{H}$ and $\mathbf{B}$.} \label{fig:f-g-h-tractable}
\end{figure}
From this form, it is not obvious that $\holts(\mathbf{G})$ and $\holts(\mathbf{H})$ are tractable.
Nor is it easy to argue why $\holts(\mathbf{F}, \mathbf{G}, \mathbf{H}, \mathbf{B})$ is tractable.
%, although the signatures seem to have some common pattern that may lead to a combinatorial argument.
%Perhaps the only obvious one is $\holts(\mathbf{F}, \mathbf{B})$, which can be reduced to a Boolean domain tractable case.

%The result of applying an 
%%
%is shown in after scaling in \cref{fig:f-g-h-tractable-after-T}.
%%%%%%%\begin{comment}
\iffalse
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
  \begin{tikzpicture}[scale=0.7]
  \node at (0, 0) {$1$};
  \node at (-1, -1) {$0$};
  \node at (1, -1) {$0$};
  \node at(-2, -2) {$0$};
  \node at (0, -2) {$0$};
  \node at (2, -2) {$0$};
  \node at (-3, -3) {$1$};
  \node at (-1, -3) {$0$};
  \node at (1, -3) {$0$};
  \node at (3, -3) {$0$};
\end{tikzpicture}
\caption{$T \teh \mathbf{F}$}
\end{subfigure}
\hspace{0.1\textwidth}
\begin{subfigure}[b]{0.3\textwidth}
  \centering
  \begin{tikzpicture}[scale=0.7]
  \node at (0, 0) {$1$};
  \node at (-1, -1) {$0$};
  \node at (1, -1) {$0$};
  \node at(-2, -2) {$0$};
  \node at (0, -2) {$0$};
  \node at (2, -2) {$-1$};
  \node at (-3, -3) {$0$};
  \node at (-1, -3) {$0$};
  \node at (1, -3) {$0$};
  \node at (3, -3) {$0$};
\end{tikzpicture}
\caption{$T \teh \mathbf{G}$}
\end{subfigure}
\\ \hfill \\
\begin{subfigure}[b]{0.35\textwidth}
  \centering
  \begin{tikzpicture}[scale=0.7]
  \node at (0, 0) {$0$};
  \node at (-1, -1) {$0$};
  \node at (1, -1) {$0$};
  \node at(-2, -2) {$0$};
  \node at (0, -2) {$0$};
  \node at (2, -2) {$0$};
  \node at (-3, -3) {$1$};
  \node at (-1, -3) {$0$};
  \node at (1, -3) {$-1$};
  \node at (3, -3) {$0$};
\end{tikzpicture}
\caption{$T \teh \mathbf{H}$}
\end{subfigure} 
\hspace{0.1\textwidth}
\begin{subfigure}[b]{0.35\textwidth}
  \centering
  \begin{tikzpicture}[scale=0.7]
  \node at (0, 0) {$0$};
  \node at (-1, -1) {$1$};
  \node at (1, -1) {$0$};
  \node at(-2, -2) {$0$};
  \node at (0, -2) {$0$};
  \node at (2, -2) {$1$};
\end{tikzpicture}
\caption{$T \tew \mathbf{B}$}
\end{subfigure}
  \caption{$\mathbf{F}, \mathbf{G}, \mathbf{H}$ and $\mathbf{B}$ after applying $T$ up to scaling} \label{fig:f-g-h-tractable-after-T}
\end{figure}
%%%%%%%%%%%%%%%%\end{comment}
\fi
% We can see that $\lvert \supp T \teh \mathbf{F} \cap \supp T \teh \mathbf{G} \rvert = 1$.
Now we apply the orthogonal transform $T = \left[ \begin{smallmatrix}
    1/\sqrt{2} & 1/\sqrt{2} & 0 \\
    1/\sqrt{2} & -1/\sqrt{2} & 0 \\
    0 & 0 & 1
\end{smallmatrix} \right]$
which transforms $\mathbf{F}, \mathbf{G}$ and $\mathbf{H}$ to be supported
in $\{\db, \dg\}^*, \{\db, \dr\}^*, \{\dg, \dr\}^*$ respectively,
%which shows that the transformed constraint functions can interact with each other only in a trivial way.
% this "shows" is not what we want to say. we want to say the theorem statement does it.
% Also, each of them can be viewed as a tractable Boolean domain function when the domain is restricted.
Their tensor decompositions  have a revealing structure. 
Ignoring the scalar constants, we have\footnote{Complex numbers do appear,  even though the signatures are all real valued. This is similar to  eigenvalues.}
\begin{align*}
    \mathbf{F}' &= T \teh \mathbf{F} = (1, 0, 0)\teh + (0, 1, 0)\teh = \mathbf{e}_1\teh + \mathbf{e}_2\teh \\
    \mathbf{G}' &= T \teh \mathbf{G} = (1, 0, i)\teh + (1, 0, -i)\teh = (\mathbf{e}_1 + i \mathbf{e}_3)\teh + (\mathbf{e}_1 - i \mathbf{e}_3)\teh \\
    \mathbf{H}' &= T \teh \mathbf{H} = (0, 1, i)\teh + (0, 1, -i)\teh = (\mathbf{e}_2 + i \mathbf{e}_3)\teh + (\mathbf{e}_2 - i \mathbf{e}_3)\teh
\end{align*}
The vectors in tensor decompositions show that geometrically, $\mathbf{F}'$, $\mathbf{G}'$, and $\mathbf{H}'$ are associated with 
three coordinate planes.
%$xy$-plane, $xz$-plane, and $yz$-plane respectively.
Written in matrix form, $\mathbf{B}' = T \tew \mathbf{B} = \left[ \begin{smallmatrix}
    0 & 1 & 0\\
    1 & 0 & 0 \\
    0 & 0 & 1
\end{smallmatrix} \right]$, with the $(i,j)$ entry being the function value $B'(i, j)$.
%This can be viewed as a transformation that swaps the $x$ axis and $y$ axis.
%Simple calculation shows that
% \begin{align*}
% (\mathbf{B}')\teh \mathbf{F}' &= \mathbf{F}' \\
% (\mathbf{B}')\teh \mathbf{G}' &= \mathbf{H}' \\
% (\mathbf{B}')\teh \mathbf{H}' &= \mathbf{G}' 
% \end{align*}
%$(\mathbf{B}')\teh \mathbf{F}' = \mathbf{F}'$,
%$(\mathbf{B}')\teh \mathbf{G}' = \mathbf{H}'$, 
%and $(\mathbf{B}')\teh \mathbf{H}' = \mathbf{G}'$.
%The fact that $\mathbf{B}'$ has finite multiplicative order, in particular $(\mathbf{B}')^2 = I$ allows us compute $\holts(\mathbf{F}, \mathbf{G}, \mathbf{H}, \mathbf{B})$ in polynomial time.
Applying  \cref{thm:dichotomy-set-of-domain-3}
we can conclude  that $\{\mathbf{F}, \mathbf{G}, \mathbf{H}, \mathbf{B}\}$ is 
tractable (in tractable class \tractBGGRBR in \cref{thm:dichotomy-set-of-domain-3}).

%%%%%% To Jin Soo: the exampe here is not to explain to the readers why it is
%%%%%% tractable. But just that it is not obvious, but covers by thm 3.1

% \section{Introduction (previous)}
% Holant problems were introduced in \cite{cai_computational_2011} as a framework of studying the computational complexity of counting problems.
% It is more expressible than the problem of counting graph homomorphisms introduced by Lov\'asz \cite{Freedman2004ReflectionPR, Hell2004GraphsAH, Lovsz1967OperationsWS}.
% The complexity classification program of counting problems is to classify the computational complexity of these problems.

% Let $\mathcal{F}$ be a set of (complex valued) constraint functions defined on some domain set $D$.
% It defines a Holant problem $\hol(\mathcal{F})$.
% An input consists of a graph $G = (V, E)$, where each $v \in V$ has an associated $\mathbf{F} \in \mathcal{F}$, with edges adjacent to $v$ corresponding to the input variables to $\mathbf{F}$.
% The output is the sum of products of evaluations of the constraint functions over all assignments over $D$ for the variables.
% The goal 
% %of the complexity classification of Holant problems 
% is to classify the complexity of $\hol(\mathcal{F})$ according to $\mathcal{F}$.
% A complexity dichotomy theorem 
% %for counting problems 
% classifies every $\mathcal{F}$ within a broad class
% %of certain restricted classes 
% to be either polynomial time solvable or \sph.


% For the classification of 
% %$\scsp$ (
% counting CSP on Boolean domain problems, much progress has been made.
% For domain size $2$, explicit dichotomy theorems have been proved, culminating in a classification of any complex valued functions \cite{Creignou1996ComplexityOG, Dyer2007TheCO, doi:10.1137/070690201, 10.1145/1536414.1536511}.
% A $\scsp$ dichotomy for a general domain also has been proven
% \cite{10.1145/2528400, Dyer2010OnTC, dyer_et_al:LIPIcs.STACS.2011.261, Cai2011ComplexityOC, 5959820}.

% On the other hand, obtaining higher domain Holant dichotomy seems far more challenging.
% Few of the existing higher domain Holant dichotomy are \cite{cai_dichotomy_2013, liu_restricted_nodate}.
% $\holts(\mathcal{F})$ is the Holant problem assuming that all unary signatures are available, i.e. $\holts(\mathcal{F}) = \hol(\mathcal{F} \cup \mathcal{U})$ where $\mathcal{U}$ is the set of all unary signatures.
% It is a natural starting point of proving dichotomy since the availability of the unary signatures make constructions easier.
% Also, as shown in \cite{cai_complexity_2017}, it can be used to prove a Holant dichotomy of more general cases.
% \cite{cai_dichotomy_2013} proves the dichotomy of $\holts(\mathbf{F})$ for a single complex valued, symmetric, ternary signature $\mathbf{F}$ on domain size $3$.
% \cite{liu_restricted_nodate} shows the dichotomy of $\holts(\mathbf{F})$ for a single $0-1$ valued, symmetric, ternary signature $\mathbf{F}$ on domain size $4$.

% In this paper, we extend the $\holts$ dichotomy on domain size $3$ of \cite{cai_dichotomy_2013} by using a result from \cite{liu_restricted_nodate} (Theorem 2 of \cite{liu_restricted_nodate}), that an exceptional form of tractable signature (form 3 in Theorem 3.1 of \cite{cai_dichotomy_2013}) does not occur when a signature is assumed to be real valued.
% By restricting ourselves to a set of symmetric, real valued signatures $\mathcal{F}$, we are able to obtain a $\holts(\mathcal{F})$ dichotomy.
% We see that the dichotomy is very closely related to the geometry of the tensor decomposition of signatures.
% Although we do not get an explicit combinatorial construction as the Fibonacci gates in the Boolean domain symmetric $\holts$ dichotomy \cite{cai_complexity_2017},
% we see that a geometric perspective can help us understand the dichotomy.


% ADD the different approach for higher arity \\
% ADD the set $\mathcal{G}$: can be viewed as the orbit of the monoid action of the binary signatures on ternary signatures, or as a gadget closure.
